Symbolic-Numeric Computation of Integrals in Successive Galerkin Approximation of Hamilton-Jacobi-Bellman Equation

This paper proposes an efficient symbolic-numeric method to compute the integrals in the successive Galerkin approximation (SGA) of the Hamilton-Jacobi-Bellman (HJB) equation. A solution of the HJB equation is first approximated with a linear combination of the Hermite polynomials. The coefficients of the combination are then computed by iteratively solving a linear equation, which consists of the integrals of the Hermite polynomials multiplied by nonlinear functions. The recursive structure of the Hermite polynomials is inherited by the integrals, and their recurrence relations can be computed by using the symbolic computation of differential operators. By using the recurrence relations, all the integrals can be computed from a part of them that are numerically evaluated. A numerical example is provided to show the efficiency of the proposed method compared to a standard numerical integration method.

==> latexmkrc <==
#!/usr/bin/perl

# How to Use ############################################################ 
# 
# For Japanese articles:
#       * Uncomment "Use platex" and comment out "Use pdflatex" in 1.
#       * Uncomment 3.
#       * Set 4. to "3"
#
# For English articles:
#       * Uncomment "Use pdflatex" and comment out "Use platex" in 1.
#       * Comment out 3.
#       * Set 4. to "1"
# 
#########################################################################

#--------------------------------------------------#
# 1. Compile Command Setting
#--------------------------------------------------#

##### Use platex (for Japanese articles) #####
#$latex = 'platex %O -src-specials -shell-escape -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

##### Use pdflatex (for English articles) #####
$latex = 'pdflatex %O -src-specials -shell-escape -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

#--------------------------------------------------#
# 2. BibTeX Setting (if you use bibtex to make references)
#--------------------------------------------------#

$bibtex = 'pbibtex %O %B -kanji=utf8';

#--------------------------------------------------#
# 3. DVI-PDF Converter Setting (if you make pdf from dvi)
#--------------------------------------------------#

#$dvipdf = 'dvipdfmx %O -o %D %S';

#--------------------------------------------------#
# 4. PDF Mode Setting
#   0: don't make pdf
#   1: use pdflatex (English)
#   2: use ps2pdf
#   3: make pdf from dvi (Japanese)
#--------------------------------------------------#

$pdf_mode = 1; 

#--------------------------------------------------#
# 5. Previewer Settings
#--------------------------------------------------#

##### Use pdf-view of tex editors #####
#$pdf_previewer = 'exit';

##### If you use external previewers (you have to verify paths of pdf previewers and tex editors) #####
##### Use SumatraPDF and VS code inverse search #####
$pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\Programs\Microsoft VS Code\Code.exe\" -g \"%f\":\"%l\"" %O %S';

##### Use SumatraPDF and Atom inverse search #####
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

#--------------------------------------------------#
# 6. Other Settings
#--------------------------------------------------#

##### Don't preserve temporary files #####
$pvc_view_file_via_temporary = 0;

#--------------------------------------------------#
# References
# * https://ichiro-maruta.blogspot.com/2016/01/atom-latex-on-windows.html
# * https://qiita.com/Rumisbern/items/d9de41823aa46d5f05a8
#--------------------------------------------------#

